HD Maps are Lane Detection Generalizers: A Novel Generative Framework for Single-Source Domain Generalization

Lane detection is a vital task for vehicles to navigate and localize their position on the road. To ensure reliable driving, lane detection models must have robust generalization performance in various road environments. However, despite the advanced performance in the trained domain, their generalization performance still falls short of expectations due to the domain discrepancy. To bridge this gap, we propose a novel generative framework using HD Maps for Single-Source Domain Generalization (SSDG) in lane detection. We first generate numerous front-view images from lane markings of HD Maps. Next, we strategically select a core subset among the generated images using (i) lane structure and (ii) road surrounding criteria to maximize their diversity. In the end, utilizing this core set, we train lane detection models to boost their generalization performance. We validate that our generative framework from HD Maps outperforms the Domain Adaptation model MLDA with +3.01%p accuracy improvement, even though we do not access the target domain images.

==> src/method.tex <==

%%%%%%%%%%%%%%%%%% 용어 통일 %%%%%%%%%%%%%%%%%%
% lane masks : lane segmentation label 전체 
% lane : 차선 하나 

\section{Methodology} 

Our framework consists total of three phases: We first introduce the lane-conditioned generation from HD Maps in~\Cref{sec:subsec:gen}. Next, we describe the core set selection criteria in~\Cref{sec:subsec:core} and training process of lane detection models in~\Cref{sec:subsec:train} 


\begin{figure*}[!t]
    \vspace{0.2cm}
    \centering
    \includegraphics[width=0.96\textwidth]{figures/main2.pdf}
    \caption{\textbf{The overall framework.} Our framework adopts HD Maps as a single-source domain to build robust lane detection models. 
    We first extract numerous lane masks from HD Maps with RGB Images. Then, we train SIS (Semantic Image Synthesis) generative models to synthesize lane-conditioned images with diverse surroundings. 
    % and project it onto the RGB images to obtain source domain data pairs of images and lane label masks. (2) A generative model is used to synthesize diverse images corresponding to the core set of lane structures with maximal diversity, selected from the source domain data. 
    Next, we select a core set among synthesized images with two criteria to maximize its diversity: \textit{(i) lane structure} and \textit{(ii) surroundings}. 
    Then, we finally train the lane detection model and obtain enhanced domain generalization performance.
    }
    \label{fig:fig2_overall_arch}
    \vspace{-2mm}
\end{figure*}

% \subsection{Preliminaries}
% We propose a framework for enhancing the generalization performance of lane detection models using HD maps and image generation models. 
% As shown in Fig.~\ref{fig:fig2_overall_arch}, we describe the proposed framework in several phases. 
% We first extract lane markings and images from HD maps and generate realistic scenes to help with training lane detection models. 
% At each phase, we try to enhance the diversity of lane structures and surroundings which we consider two main factors for domain discrepancy in lane detection. 


\textbf{Problem Statement.}
For the Single-Source Domain Generalization (SSDG) for lane detection, we use source domain ${D_s}$ which consists of pairs of driving environment images and lane masks. 
Notably, our work demonstrates HD Maps provide a successful source for mitigating domain discrepancy in lane detection situations. 
To train the lane detection model as robustly as possible to the unseen target domains ${D_t}$, we propose a diversity-aware framework by selecting a core set. 
% Specifically, we extract the core set ${D_s^*}$ of augmented samples maximizing the diversity of surroundings and lane structures. 
%which are aforementioned for the factor of domain discrepancy. 


\subsection{Lane-conditioned Generation from HD Maps}\label{sec:subsec:gen}

% We first target to generate lane-conditioned images from HD Maps. 
We note that the huge potential of HD Maps is the flexibility of extracting diverse lane labels by only camera parameters. 
Using the camera parameters of pre-built HD Maps, we extract the lane label masks by projecting the lane objects in HD Maps onto the camera image plane within the camera view at the current location. 
It is worth noting that this process does not require any additional annotation to obtain the pixel-wise label of the lane markings. 
With this projection, we acquire a substantial number of lane-label masks from HD Maps easily.
Next, utilizing these lane-label masks, we adopt Semantic Image Synthesis (SIS) methods~\cite{sushko2020you, wang2018high} to generate lane-conditioned images. 
Unlike conventional SIS approaches, we use only lane labels to generate images with diverse surroundings. 


\subsection{Coreset Selection to boost Diversity}\label{sec:subsec:core}

We now introduce our coreset selection method to boost the diversity of single-source domain. 

\textbf{Data Selection Policy.}  
We first define \textit{maximal diversity} as \textit{minimum sum of similarities} between nodes in a graph.
Let's assume a complete weighted graph $G=(V, E, W)$ where the vertex set $V=\{v_1, v_2, ..., v_N\}$ represents $N$ data points, and each data point is connected to every other data point through an edge $E=\{(v_i, v_j)\}$. The weight of each edge $W=\{w(i,j)\}$ is defined as the similarity between the two data points connected by the edge. The near-optimal solution can be configured as Algorithm~\ref{alg:search_algo}.   % 방법론 
This is freely applied to various types of data by defining only a simple metric, so it is easily expanded to both lane structure and surrounding image.   % 우리 방법에 좋은 이유 
Next, we define two similarity criteria for \textit{(i) lane structure} and \textit{(ii) surroundings} to achieve maximal diversity selection.


\textbf{\textit{(i) Criteria of Lane Structure}.} 
We propose a lane similarity function $s$ between two lane label masks $\textbf{M}_i, \textbf{M}_j$ that can take into account the number of lanes and curvature. 
We first simplify the problem by defining the similarity between the projections of each lane mask $\ell$ onto the image plane. We plan to use the method proposed by \cite{eigenlane} to compare the similarity between lane curves represented in pixel coordinates. 
% 여기에 eigenlane 장점 들어가면 좋을 듯? 

First, we express a lane as a set of 2D points uniformly sampled along the vertical direction in the image plane, i.e., $\ell=[x_1, x_2, ..., x_N]^T$, where $x_i$ denotes the $x$-coordinate of the $i$-th sample, and $N$ is the number of samples. 
We construct a lane matrix $\textbf{A}=[\ell_1, \ell_2, ..., \ell_L]$ by utilizing all $L$ lane curves from the entire training data. By applying the SVD algorithm to the constructed lane matrix $\textbf{A}$, we can factorize it as follows:
\begin{equation}
   \textbf{A}= \textbf{U} \Sigma \textbf{V}^T,
\end{equation}
where $\textbf{U}=[\textbf{u}_1, ..., \textbf{u}_N]$ and $\textbf{V}=[\textbf{v}_1, ..., \textbf{v}_L]$ are orthogonal matrices, and $\Sigma$ is a singular value matrix. 
Therefore, each lane curve $\ell$ can be approximated using $M$-rank approximation with singular vectors $\textbf{u}_1, ..., \textbf{u}_M$ as follows:
\begin{equation}
\tilde{\ell_i} = \textbf{U}_M \textbf{c}_i = [\textbf{u}_1, ..., \textbf{u}_M] \textbf{c}_i.
\end{equation}

The coefficient vector $\textbf{c}_i$ of each lane curve $\ell_i$ in the \textit{eigenlane} space spanned by the singular vectors $[\textbf{u}_1, ..., \textbf{u}_M]$ can be expressed as follows:
\begin{equation}
\textbf{c}_i = \textbf{U}_{M}^{T} \ell_i = [c_1, ..., c_M].
\end{equation}

Therefore, we simply define the similarity between two lane curves $\ell_i$ and $\ell_j$ as Euclidean distance by projecting onto the \textit{eigenlane} space as follows:
\begin{equation}
d(\ell_i, \ell_j) = | \textbf{c}_i - \textbf{c}_j |.
\end{equation}

Our goal is to extend the similarity between lane curves to between lane label masks.
Given two lane label masks $\textbf{M}_i=[\ell_{0}^{i}, ..., \ell_{m}^{i}]$ and $\textbf{M}_j=[\ell_{0}^{j}, ..., \ell_{n}^{j}]$, each containing $m$ and $n$ lane curves, respectively.
Assuming that $m\ge n$ always holds, we define the lane layout similarity $s$ between lane label marks $\textbf{M}_i, \textbf{M}_j$ as follows: 
\begin{equation}
  s(\textbf{M}_i, \textbf{M}_j) = \sum^{n}_{k} \min_{l}  d( \ell_{l}^{i}, \ell_{k}^{j} )  + |m-n|~\kappa,
\end{equation}
where $\kappa$ denotes the penalty constant which we describe next. 
We believe that the number of curves is also an important factor in determining the similarity. 
Therefore, when the two-lane label masks have different numbers of lane curves, we penalize their similarity by adding $\kappa$.
We empirically determine the penalty constant $\kappa$ from the training dataset.
This indicates that we consider the number of lane curves to be an important factor affecting diversity in most cases. With the definition of similarity between lane label masks, we can select the $K_{\text{scene}}$ number of masks that maximize the diversity of lane layouts by using the selection algorithm in Algorithm~\ref{alg:search_algo}.

\begin{algorithm}[t]
% \footnotesize 
\small
% \caption{Finding a set of K vertices \newline with the minimum sum of similarity}
\caption{Data Selection Policy}
\begin{algorithmic}[1]
\Require Complete weighted graph $G$ and $K=\#$ of vertices
\State Find the vertex pair $(i,j)$ which has minimum $w(i, j)$
\State Add $i$ and $j$ to $Q$
\While{$|Q| < K$}
\State Find vertex $k$ which minimizes $\sum_{l \in V \setminus Q} w(k, l)$
\EndWhile
\Ensure $Q$
\end{algorithmic}
\label{alg:search_algo}
\end{algorithm}


% \subsection{(ii) Criteria of Road Surroundings}

% \subsection{Increasing the diversity of surroundings}
% \textbf{Image scene extraction from HD map.}     % image extraction..? 

\textbf{\textit{(ii) Criteria of Road Surrounding}.}
We expect that by training the model with RGB images having identical lane labels, but different surroundings and backgrounds, the model will be less sensitive to changes in the backgrounds and surroundings. 
However, unlike the case of lane layouts, it is difficult to obtain a quantitative measure of the similarity between backgrounds or surroundings in RGB images. 
Therefore, we adopt a comparison metric commonly used to check the quality of generated images by image synthesis models.
% Therefore, we define the similarity of the surroundings in RGB images as an image metric. 

The Structural Similarity Index Measure (SSIM)~\cite{ssim} and its Multi-Scale extension (MS-SSIM)~\cite{ms-ssim} are common metrics to evaluate the perceived quality or similarity of images.  
% They are commonly used for measuring the similarity between two images. 
% Recently, MS-SSIM has also been used to compare the quality of generated images against the reference images in image generation tasks~\cite{snell2017learning}. 
Since MS-SSIM has also been used to compare the quality of generated images against the reference images in image generation tasks~\cite{snell2017learning}, we choose the MS-SSIM as the similarity metric between two generated images.     
We generate 100 RGB images for each lane label mask and we selected $K_{\text{image}}$ most perceptively diverse set of generated images using MS-SSIM and the method described in Algorithm~\ref{alg:search_algo}.

\subsection{Training Lane Detection Model with Coreset}\label{sec:subsec:train}

Combining selections from both lane structure and surrounding, we build the coreset which maximized diversity. Please note that this coreset is originally from HD Maps. 
Then, we finally train the lane detection model using this dataset. 
It is noteworthy that our framework is model-agnostic, which means it applies all lane detection models like augmentation.  

% Finally, to train the lane detection model, 




==> src/related.tex <==
% < 1. Domain Adaptation w/ Lane Detection > - O 


\section{Related Works}

\subsection{Domain Adaptation for Lane Detection} 
Unsupervised Domain Adaptation(UDA)~\cite{uda1,uda2,uda3,uda4} has been primarily adopted as a methodology for bridging domain discrepancy that occurs between different domains. In fact, it allows access to unlabeled target domains in the model learning process. Current research for domain adaptation in lane detection can be largely categorized into (i) Sim-to-Real and (ii) Cross-domain adaption. 

(i) \textbf{Sim-to-Real domain adaptation} is a field that adapts simulated data generated by gaming engines to the real world. Their main goal is to bridge the domain gap between photorealistic synthetic images and real-world data. ADA~\cite{simada} utilizes adversarial discriminative and generative methods for adapting to the target domain, and UNIT~\cite{simunit} utilizes cycle-GAN-based methods. 

(ii) \textbf{Cross-domain adaptation} is a method for narrowing the domain gap that occurs in two different driving environments. MLDA~\cite{li2022multi} is the first paper to point out the cross-domain discrepancy among CULane and TUSimple datasets. They solve this domain gap with a framework based on self-training.
In particular, the setting of MLDA is also a form of cross-evaluation with only one source domain. However, the biggest difference from our framework is that they use RGB images of the target domain in their adaptation process.

Given that both of the above fields require target domain information, it is difficult to apply it in a realistic driving environment.

% < 2. Single-Source Domain Generalization > 
\subsection{Single-Source Domain Generalization} 
Unlike Multi-Source Domain Generalization(MSDG), Single-Source Domain Generalization(SSDG)~\cite{ssdg1,ssdg2,ssdg3} utilizes only one source domain during training. Intuitively, SSDG is more difficult to generalize successfully than MSDG because of the limited training situations. 
Existing SSDG models have been developed by applying data augmentation techniques to the source domain and expecting to make a robust dataset~\cite{su2023rethinking,wang2021learning,volpi2018generalizing,qiao2020learning}. 
The landmark works are ADA~\cite{volpi2018generalizing} and M-ADA~\cite{qiao2020learning}, which use adversarial data augmentation techniques to conduct pixel-level additive perturbation. 

On top of that, the maximization of diversity has been widely explored to boost generalization effects.~\cite{wang2021learning,wacv23diverse,zhang2019adversarial,hendrycks2019augmix, yun2019cutmix} % citation
ALT~\cite{wacv23diverse} produces diverse images using a separate diversity module that combines augmentation such as Augmix~\cite{hendrycks2019augmix} and RandConv~\cite{randconv}.
However, from the standpoint of lane detection fields, these augmentation techniques are insufficient to contain a complex and dynamic driving environment. Therefore, in this work, we propose a method of selecting a core set that can maximize the diversity of lane structures and surroundings for generalizing lane detection models.
%as part of a more advanced augmentation method.



% < 3. HD map > -> \daeun{HDmap의 background / lane structure에서의 장점이 추가되면 좋을 것 같다.}
\subsection{HD maps}     
HD maps are widely recognized for their ability to provide accurate and detailed semantic information about road environments in a machine-readable form.
Despite being represented in a lightweight vector map format, HD maps contain detailed and accurate information about the road environment. 
This information is primarily used for vehicle localization and control~\cite{hdmap_loc}. 
Recently, there has been a growing interest in the rich semantic information contained in HD maps, and several studies~\cite{hdmap_trajpred, hdmap_cd2, hdmap_gen1} have utilized them for various other tasks beyond localization and control. 
Similarly, our study also utilizes road information from HD maps to improve the generalization performance of lane detection. 

==> src_icra/conclusion.tex <==
\section{Conclusion}
We propose a novel training framework that utilizes HD maps for robust lane detection. We generated a large number of images from HD maps with varying surroundings and lane structures to mitigate domain discrepancy on lane detection. Training the lane detection model with these datasets resulted in improved generalization performance. 
Our extensive experiments successfully demonstrate this improvement and we expect our method can be fully extended on autonomous driving scenarios.

==> src_icra/exp.tex <==
% main table

\section{Experiments} 


\begin{table*}
\vspace{0.3cm}
\centering
\renewcommand{\arraystretch}{1.35}
\setlength{\tabcolsep}{.45em}    %45
    \caption{\textbf{Quantitative comparison results on CULane}.
    We evaluate the generalization performance on CULane from TUSimple and LabsLane respectively. 
    % Since there are no lane markings in the image, we measure the FP score for Crossroad.
    \dag Note that we attempted to reproduce ~\cite{li2022multi}, but were not even able to reproduce their baseline, "Source only". Therefore, in this table, we present their results as they are reported.
    }
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l|ccc|cccccccccc}
    \hline
    \multicolumn{1}{c|}{\multirow{2}{*}{Experiment setting}} & \multicolumn{3}{|c|}{Trained data} & \multirow{2}{*}{Total} & \multirow{2}{*}{Normal} & \multirow{2}{*}{Crowded} & \multirow{2}{*}{Night} & \multirow{2}{*}{No line} & \multirow{2}{*}{Shadow} & \multirow{2}{*}{Arrow} & \multirow{2}{*}{Dazzle light} & \multirow{2}{*}{Curve} & \multirow{2}{*}{Crossroad} \\ \cline{2-4}
    
    \multicolumn{1}{c|}{} & TUSimple & CULane & LabsLane &  &  &  &  &  &  &  &  &  &  \\ \hline\hline
    
    Source only - ERFNet & \ding{52} &  &  & 24.2 & 41 & 19.6 & 9.1 & 12.7 & 12.7 & 28.8 & 11.4 & 32.6 & 1240 \\
    Source only - GANet & \ding{52} &  &  & 30.5 & 50 & 25.5 & 19.6 & 18.5 & 16.8 & 36 & 25.4 & 34.2 & 7405 \\ 
    Source only - GANet &  &  & \ding{52} & 34.9 & 52.4 & 25.9 & 27.1 & 18.8 & 20.3 & 44.5 & 25.9 & 42.7 & \textbf{939} \\  \hline
    % Target only - GANet &  & \ding{52} &  & 78.8 & 93.2 & 77.2 & 72.8 & 53.6 & 77.9 & 89.6 & 71.2 & 75.9 & 1240 \\ \hline
    % Augmix & \ding{52} &  &  &  &  &  &  &  &  &  &  &  &  \\
    % Cutmix & \ding{52} &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
    Advent~\cite{advent} & \ding{52} & \ding{52} &  & 30.4 & 49.3 & 24.7 & 20.5 & 18.4 & 16.4 & 34.4 & 26.1 & 34.9 & 6527 \\
    PyCDA~\cite{pycda} & \ding{52} & \ding{52} &  & 25.1 & 41.8 & 19.9 & 13.6 & 15.1 & 13.7 & 27.8 & 18.2 & 29.6 & 4422 \\
    Maximum Squares~\cite{maximum} & \ding{52} & \ding{52} &  & 31 & 50.5 & 27.2 & 20.8 & 19 & 20.4 & 40.1 & 27.4 & 38.8 & 10324 \\
    MLDA~\cite{li2022multi}\dag & \ding{52} & \ding{52} &  & \underline{38.4} & \textbf{61.4} & \textbf{36.3} & \underline{27.4} & \underline{21.3} & \textbf{23.4} & 49.1 & \underline{30.3} & \underline{43.4} & 11386 \\ \hline
    {\cellcolor[HTML]{EFEFEF}Ours - ERFNet} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}\ding{52} & \cellcolor[HTML]{EFEFEF}38.2 & \cellcolor[HTML]{EFEFEF}\underline{56.8} & \cellcolor[HTML]{EFEFEF}32.5 & \cellcolor[HTML]{EFEFEF}24.4 & \cellcolor[HTML]{EFEFEF}\textbf{23.8} & \cellcolor[HTML]{EFEFEF}\underline{22.3} & \cellcolor[HTML]{EFEFEF}\underline{51.2} & \cellcolor[HTML]{EFEFEF}\textbf{32.2} & \cellcolor[HTML]{EFEFEF}40.9 & \cellcolor[HTML]{EFEFEF}4572 \\
    {\cellcolor[HTML]{EFEFEF}Ours - GANet} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF} & \cellcolor[HTML]{EFEFEF}\ding{52} & \cellcolor[HTML]{EFEFEF}\textbf{39.6} & \cellcolor[HTML]{EFEFEF}56.7 & \cellcolor[HTML]{EFEFEF}\underline{34} & \cellcolor[HTML]{EFEFEF}\textbf{30.1} & \cellcolor[HTML]{EFEFEF}21.2 & \cellcolor[HTML]{EFEFEF}22 & \cellcolor[HTML]{EFEFEF}\textbf{53.2} & \cellcolor[HTML]{EFEFEF}27.1 & \cellcolor[HTML]{EFEFEF}\textbf{46.9} & \cellcolor[HTML]{EFEFEF}\underline{1275} \\ \hline
    \end{tabular}%
    }
    \label{ref:table_qualitative_result}
\end{table*}

\subsection{Datasets}
In this paper, we use three datasets for SSDG settings: 
LabsLane HD maps were used as the single source domain, and two commonly used benchmarks CULane and TUSimple were used as the target domain.

\textbf{LabsLane:} We used Naver Labs HD map\footnote{https://naverlabs.com/en/datasets} to create the lane label masks, which are publicly available for research purposes and provide rich information about the road environment in cities of South Korea.
In order to obtain RGB images, we utilized mobile mapping vehicles equipped with high-precision RTK GPS to collect more than 100,000 images.
During the projection of the lane object onto the camera view, we only considered a maximum of four lanes near the ego vehicle, which is consistent with other benchmark datasets that also have a maximum of four or five lanes.
To maximize the diversity of lane layouts, we selectively sampled only the data that exhibited minimum similarity and removed duplicates.
% Moreover, to exclude cases where all lanes are occluded by excessive moving obstacles, we utilized a semantic segmentation algorithm~\cite{cheng2022masked}.
As a result, the generated dataset, called LabsLane, consists of 7,184 RGB images and corresponding 6 DoF poses.

\textbf{CULane:} It consists of complex \textit{urban road environments} and 133,235 frames, of which 88,880, 9,675, and 34,680 are used for training, validation, and testing, respectively. 
% The test set is divided into a normal class and eight challenging classes, including crowded, night, no line, shadow, arrow, dazzle light, curve, and crossroad.

\textbf{TUSimple:} It mostly consists of \textit{highway} driving scenes and around 7,000 video clips, each containing 20 frames, with labeled lanes on the final frame of each clip.


\subsection{Implementation details}
\textbf{Training:}
To implement the proposed framework, we used Semantic Image Synthesis(SIS) models like OASIS~\cite{sushko2020you} and Pix2PixHD~\cite{wang2018high} as generative models. Note that since we wanted to generate diverse surroundings from lane masks extracted from HD maps, we used only lane labels without using the entire semantic label like conventional SIS models. 

Also, we used GANet-small~\cite{wang2022keypoint} and ERFNet~\cite{romera2017erfnet} as lane detection models which are respectively keypoint-based and segmentation-based. We tried to validate the versatility of our method in various types of lane detection models.
To ensure a fair comparison, when we used ERFNet~\cite{romera2017erfnet}, we followed the settings of benchmark datasets proposed by the domain adaptation method, MLDA~\cite{li2022multi}.
For instance, we adopted the pre-processing method proposed in MLDA when using ERFNet, which established experimental settings for the generalization of lane detections.
For each model, we followed their default settings during training. 
Specifically, all images in each dataset were resized to $768\times256$ to unify the size of both dataset, and only 1-degree rotation was used for augmentation.

\textbf{Evaluation:}
We used the official evaluation code provided by CULane and TUSimple. 
Also, we use F1 score and accuracy respectively to measure the performance metric for CULane and TUSimple. 

\begin{table}[t!]
\centering
\caption{\textbf{Quantitative results on TUSimple dataset.} We evaluate the generalization performance on TUSimple from CULane and LabsLane respectively. Note that our framework using LabsLane shows similar performance with Target only.}
\label{tab:ablation_study}
\renewcommand{\arraystretch}{1.35}
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{l|ccc|ccc}
    \hline
    \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{Trained data} &  &  &  \\ \cline{2-4}
    \multicolumn{1}{c|}{\multirow{-2}{*}{Experiment setting}} & CULane & TUSimple & LabsLane & \multirow{-2}{*}{Acc} & \multirow{-2}{*}{FP} & \multirow{-2}{*}{FN} \\ \hline\hline
    Source only - ERFNet & \ding{52} &  &  & 60.9 & 31.6 & 55.2 \\
    Source only - GANet & \ding{52} &  &  & 76.9 & {\ul 25.8} & 35 \\ 
    Target only - GANet &  & \ding{52} &  & 95.9 & 1.97 & 2.62 \\ \hline
    Advent~\cite{advent} & \ding{52} & \ding{52} &  & 77.1 & 39.7 & 43.9 \\
    PyCDA~\cite{pycda} & \ding{52} & \ding{52} &  & 80.9 & 51.9 & 45.1 \\
    Maximum Squares~\cite{maximum} & \ding{52} & \ding{52} &  & 76 & 38.2 & 42.8 \\
    MLDA~\cite{li2022multi} & \ding{52} & \ding{52} &  & {\ul 89.7} & 29.5 & {\ul 18.4} \\ \hline
    \rowcolor[HTML]{EFEFEF} 
    % Ours - ERFNet &  &  & \ding{52} &  &  &  \\
    \rowcolor[HTML]{EFEFEF} 
    Ours - GANet &  &  & \ding{52} & \textbf{92.4} & \textbf{6.7} & \textbf{9.4} \\ \hline
    \end{tabular} %
    }
    \label{ref:table_tusimple}
    \vspace{-0.4cm} 
\end{table}

\subsection{Quantitative results}
\textbf{Results on CULane:}    
In Table \ref{ref:table_qualitative_result}, we summarize the performances of each lane detection model on CULane dataset, which includes various scenario cases. 
We compared our methods with domain adaptation methods such as Advent~\cite{advent}, PyCDA~\cite{pycda}, Maximum Squares~\cite{maximum}, and MLDA~\cite{li2022multi}. ERFNet~\cite{romera2017erfnet} was used for testing all of the above methodologies.

Although our approach is an SSDG approach, we observe that our total performance outperforms MLDA.
In particular, the performance improvement was greater when it was not a typical surrounding scene (e.g. Night, Dazzle light). 
% Furthermore, in the case of curve lanes which are different from typical lane structures, the range of performance improvement was remarkable. 
This demonstrates that our HD map-based diversity maximization framework can robustly handle large domain shifts.

\textbf{Results on TUSimple:}
We also validated our proposed framework on the TUSimple dataset in Table~\ref{ref:table_tusimple}.
We found that our proposed framework outperforms the domain adaptation-based methods even though we do not use target domain information.
It is especially notable that both MLDA~\cite{li2022multi} and the proposed method showed significant performance improvements compared to the results on CULane dataset.
We conjecture that since CULane dataset is more diverse than TUSimple, it benefits more from the diversity-enhancing stages of our proposed framework.


\subsection{Ablation studies}

\textbf{Using benchmark images instead of HD maps:}    
We also conducted experiments on benchmark images rather than HD maps to verify the efficacy of our training framework itself. 
We measured the performance of the model learned from TUSimple to CULane.
Note that it is different from MLDA~\cite{li2022multi} setting which targets Domain Adaptation scenario. 
As shown in Table~\ref{ref:tu2cu}, our framework outperforms the source-only model, especially when our selection method is employed. Also, note that the performance increased for both Pix2pix and OASIS. We expect any semantic image synthesis model can be easily utilized in our framework

%We observed the framework using our generative model improves the Source-only performance with any generative model like Pix2pix~\cite{wang2018high} or OASIS~\cite{sushko2020you}. We also expect any other semantic image synthesize models to be easily utilized with our framework. 
% As shown in Table~\ref{ref:tu2cu}, our framework also performs well on the benchmark dataset.

\begin{figure}[!]
    \vspace{0.2cm}
    \centering
    \includegraphics[width=0.28\textwidth]{figures/graph.png}
    \caption{
    \textbf{Effect of the number of selected data}.
    We compare the performance of randomly selecting 10 data from 100 images generated from a single lane label mask and selecting 2, 5, and 10 data using the proposed diversity-aware image selection method.
    }
    \label{fig:efficacy_selection}
\end{figure}



\textbf{Effect of the number of selected images:}
We also experimented with the efficacy of the number of selected images.
We used accuracy and total F1-score as comparison metrics for TUSimple and CULane datasets, respectively.
In Fig.~\ref{fig:efficacy_selection}, we compare the performance of randomly selecting 10 samples from a single lane label mask of LabsLane dataset with selecting 2, 5, and 10 samples using the proposed diversity-aware image selection method.
The figure shows that the proposed selection method generally outperforms random selection, and the performance is the highest when selecting 5 data for each lane label.
Therefore, we set the number of synthesized data $K_{image}$ to 5 for all experiments.


\begin{table}[t!]
\centering
\renewcommand{\arraystretch}{1.3}
\begin{adjustbox}{width=0.4\textwidth}
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{lccc}
    \hline
    \multicolumn{1}{c}{} & Total & Normal & Curve \\ \hline
    Source only (TUSimple) & 24.1 & 41 & 32.6 \\ \hline
    Pix2pix~\cite{wang2018high} & 26.7 & 43 & 33.2 \\
    OASIS~\cite{sushko2020you} & 27.3 & 45 & 37.3 \\
    \rowcolor[HTML]{EFEFEF} 
    OASIS + Our selection method & \textbf{31.2} & \textbf{47.9} & \textbf{40.4} \\ \hline
    \end{tabular}%
    }
    \end{adjustbox}
\caption{\textbf{Evaluating our methods using TUSimple images.} To verify the versatility of our framework, we tested our framework on benchmark dataset.}
\label{ref:tu2cu}
\vspace{-.4cm}
\end{table}

\textbf{Using other image synthesis model:}
We also validated that our proposed framework works well with other image synthesis models.
We used Pix2PixHD~\cite{wang2018high}, another algorithm that can generate diverse images by re-sampling noise vectors. 
We trained the image synthesis model on TUSimple and evaluated the performance on total F1-score of CULane. 
As shown in Table~\ref{ref:tu2cu}, we observed a performance improvement of about 10\% when using Pix2PixHD~\cite{wang2018high} compared to training on TUSimple.
However, we believe that the reason for the difference in performance is due to the quality of the generated images, as OASIS~\cite{sushko2020you} produced more realistic images compared to Pix2PixHD~\cite{wang2018high}. 


\begin{figure}[t!]
    \vspace{0.2cm}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/exp_figs.pdf}
    \caption{\textbf{Examples of generated dataset.} We utilized OASIS as our generative model to visualize results. Our diversity maximization framework effectively helped with generating diverse surroundings.
    }
    \label{fig:fig3_examples}
    % \vspace{-2mm}
\end{figure}

\subsection{Discussions}

\begin{table}[t!]    
    \centering
    \renewcommand{\arraystretch}{1.3}
    \begin{adjustbox}{width=0.3\textwidth}
    \resizebox{\columnwidth}{!}{%
        \begin{tabular}{l|cc|c}
        \hline
        \multicolumn{1}{c|}{} & \multicolumn{2}{c|}{Source domain} &  \\
        \multicolumn{1}{c|}{\multirow{-2}{*}{}} & Simulator & HD map & \multirow{-2}{*}{Acc} \\ \hline
        UNIT~\cite{simunit} & \ding{52} &  & 77.5 \\
        MUNIT~\cite{simmunit} & \ding{52} &  & 78.6 \\
        ADA~\cite{simada} & \ding{52} &  & 82.9 \\ \hline
        \rowcolor[HTML]{EFEFEF} 
        Ours &  & \ding{52} & \textbf{92.4} \\ \hline
        \end{tabular}%
    }
    \end{adjustbox}
\caption{\textbf{Results on TUSimple compared to Sim-to-Real domain adaptation.} Our performance outperforms the existing Sim-to-Real DA performance without taking advantage of any information from TUSimple.}
\label{ref:sim2ours}
\vspace{-.4cm}
\end{table}

\textbf{Comparison with Sim-to-Real adaptation method:} 
The framework using HD map can be regarded as similar to the simulator in that it generates diverse augmented data. Therefore, we compared the performance on TUSimple with existing Sim-to-Real domain adaptation models~\cite{simunit, simmunit, simada} in Table~\ref{ref:sim2ours}. 
Their photo-realistic source domain was made by CARLA~\cite{simcarla} which is a gaming engine to generate synthetic datasets. 
Note that, UNIT~\cite{simunit}, MUNIT~\cite{simmunit}, and ADA~\cite{simada} models included TUSimple's unlabeled image as they are domain adaptation works. However, our result outperforms the existing Sim-to-Real DA performance without taking advantage of any information from TUSimple.

\textbf{Comparison with cross-domain adaptation method:} 
In Table \ref{ref:table_qualitative_result}, we compared the proposed framework with domain adaptation methods. 
% Since MLDA~\cite{li2022multi} was trained on a different lane detection model (ERFNet~\cite{romera2017erfnet}), we also re-evaluated the proposed framework based on the same lane detection model for a fair comparison.
We confirmed that our proposed framework shows comparable results with MLDA even without any knowledge of the target domain. 
Furthermore, we believe that the proposed framework is not limited to a specific lane detection model but can be applied to other various lane detection models as well.

% \textbf{Social impact:}
% As our model is about building more reliable autonomous driving systems, our work would inherit its social impact. Our framework is free from the legal data use problem by generating autonomous driving data through models.
% In addition to improving generalization performance, we believe that the proposed framework can be easily extended to domain adaptation, using data from the target domain.
% By training the image generation model on target domain data, our framework can be naturally used as a new augmentation method for the target domain.




==> src_icra/intro.tex <==
\section{Introduction}


%% MH:: 전반적으로 우리가 제안한? 용어 (lane structures라든가 surroundings라든가)들의 통일이 필요해보임

%% < Lane detection task에 대한 일반론 >
%% 다만 우리가 태클하려는 문제는 classical method에서는 나타나지 않는 문제일 수도 있음
%% 따라서 현재 lane detection algorithm이 대부분 learning-based을 기반으로 한다고 언급할 것
Lane detection is a fundamental task in autonomous driving. 
By detecting lane markings on the road, autonomous vehicles can localize their position and identify drivable spaces, which provide fundamental information for safe operation on the road. 
Recently, thanks to advancements in deep learning, most studies have shifted from using traditional hand-crafted features to employing a data-driven approach, such as deep neural networks.
%Unlike classical methods that rely on characteristic lane markings, recent advancements in deep learning have enabled data-driven approaches, which have consistently outperformed their predecessors in various benchmark evaluations. % MH:: 뒷문단 첫문장이랑 너무 겹치는 것 같은데

%% < data-driven lane detection 방법의 문제 제기 >
%% 일반적인 Normal scene에 비해서 (차선의 수가 변할 때)라든가 (심각한 background의 변화가 존재할 때) 더 크게 감소한다 
%% -> 그래서 우리는 (차선의 수)와 같은 lane의 structure와 (background의 변화를 표현하는) surrounding으로 문제를 나눠서 divide-and-conquer 할 것임 (이라고 나중에 서술할 수 있도록 밑밥)
Nevertheless, data-driven lane detection algorithms still suffer from a performance degradation when tested on unseen or out-of-distribution data.
The fundamental assumption of the data-driven approach is that the target data follows similar statistics to the training data~\cite{qiao2020learning}. 
As demonstrated in Fig.~\ref{fig:intro} (a), however, lane detection datasets typically vary due to various factors, such as camera mounting positions, road widths, capture times, and even country-specific lane marking standards.
Such discrepancies between the source and target datasets result in a severe performance decrease as shown in Fig.~\ref{fig:intro} (b).
Notably, we observed that the performance decrease between datasets is more noticeable not only when lane structures change (e.g., no lanes or curves) but also during transitions like day-to-night shifts, which notably impact the background surroundings compared to typical scenes. %(Normal).

% As shown in Figure~\ref{fig:intro}, 
% the state-of-the-art lane detection algorithm~\cite{wang2022keypoint}
% exhibits distinct performance differences depending on the training datasets.
% A domain discrepancy can arise between datasets acquired in different environments, attributed to various factors, including camera mounting positions, road widths, capture times, and even country-specific lane marking standards.
% Typically, the domain discrepancy between datasets results in a decrease in performance.
% Significantly, this performance degradation is more pronounced not only when lane structures change (e.g., no lanes or curves) but also during transitions like day-to-night shifts, affecting the background surroundings compared to typical scenes (Normal).
%where state-of-the-art lane detection models~\cite{wang2022keypoint} experience a sharp drop in performance when evaluated on different benchmark datasets they were not specifically trained on. 
% Especially, significant performance degradation
% occurs not only when lane structures change (e.g., no lane or curves) but also during day-to-night transitions (Night) compared to general scenes (Normal). 
% This highlights that lane detection algorithms are also influenced by the surrounding environment. % 문장 너무 구림
%This drop in performance becomes even more pronounced in general scenes with abrupt background changes, such as day-to-night transitions, and when the number of lanes differs between datasets.
%% MH:: (Fig 1(b)도 Normal / Curve / Night / No lane 으로 나눠서 4 column으로 구성할 것)
% -> DE :: 넵 수정하겠습니다!! 

% \begin{figure}[!]
%     \centering
%     \subfloat[]{\includegraphics[width=0.49\linewidth]{./figures/fig1a.pdf}}
%     \subfloat[]{\includegraphics[width=0.49\linewidth]{./figures/fig1b.pdf}}
%     \caption{\textbf{Performance degradation by domain discrepancy.} 
%     (a) Example images of source and target domains and
%     (b) performance of the state-of-the-art lane detection model~\cite{wang2022keypoint} on the target domain, still revealing significant challenges due to domain differences.    
%     % (b) We observed severe performance degradation in various scenes due to the domain discrepancy. All of the performance was measured from GANet~\cite{wang2022keypoint}. 
%     % (b) In fact, the difference between the two datasets exists in surroundings and lane structures
%     }
%     \label{fig:intro}
%     %% MH:: figure에 들어있는 글자 크기 더 키우기 -> DE :: 넵 수정하겠습니다!! 
%     %%      caption 수정하겠음
%     \vspace{-0.3cm}
% \end{figure}

\begin{figure}[t!]
    \vspace{0.2cm}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/fig1_v2.pdf}
    \caption{\textbf{Performance degradation by domain discrepancy.} 
    (a) Example images of source and target domains and
    (b) performance of the state-of-the-art lane detection model~\cite{wang2022keypoint} on the target domain, still revealing significant challenges due to domain differences. 
    }
    \label{fig:intro}
    % \vspace{-2mm}
\end{figure}


%% < 왜 DA / DG같은 일반적인 방법을 쓰지 않는 가 >
%% 일반적으로 다른 task에서 이런 domain discrepancy가 발생했을 때 사용하는 DA나 DG 방법론은 lane detection과 잘 맞지 않는다고 우기자
%% (좀 더.. DA/DG나 우리와 같은 lane detection의 characteristic을 분석한 방법의 차이를 결정짓도록 말하고 싶은데)
Recent studies~\cite{dg1,dg2,dg3,dg4,dg5} have attempted to address this performance degradation by incorporating additional data.
These approaches include domain adaptation, which involves making use of a limited number of data samples from the target domain, and domain generalization, which leverages data from multiple source domains.
However, in realistic autonomous driving scenarios, it is technically impossible to obtain even a small number of data samples from the target domain, as the target domain cannot be predetermined. 
Additionally, collecting data from numerous regions may have practical limitations.
Therefore, for the lane detection task, it is essential to achieve generalization solely relying on a single-source domain without any prior information about the target domain.

% These approaches include domain adaptation where target domain data is used or multiple source domains are employed for domain generalization. 
% However, obtaining data for the target region in advance is physically impossible, and collecting data from numerous regions may have practical limitations. 
% Therefore, to address realistic autonomous driving scenarios, it is essential to achieve generalization solely relying on a single-source domain without any prior information about the target dataset.


%% < SSDG 문제에서 diversity의 중요성 / 현실적인 데이터 취득의 어려움 >
%% intro에서는 상황/문제 제기까지만 하는 걸로 하자
%% 그래서 우리는 어떻게 해결했는가에 대한 궁금증만 남기자

%In the context of the Single-Source Domain Generalization (SSDG) problem, it is imperative to enhance diversity solely using the source domain (citation). 
In the context of single-source domain generalization (SSDG), it is imperative to obtain domain-invariant features, which necessitates a sufficiently diverse set of source domain data. 
Furthermore, controlling the augmentation of diversity within a constrained dataset helps the model concentrate on task-specific features.
For instance, if there are data pairs with identical surrounding conditions (background, weather, obstacles, etc.) but varying lane structures, it is conceivable that the model will be trained to progressively disregard the influence of the surroundings.
However, unfortunately it is practically impossible to acquire data with different lane structures while maintaining the same surrounding conditions.


% \begin{figure}[!]
%     % \centering
%     \includegraphics[width=0.5\textwidth]{figures/ssdg_fig2_v2.eps}
%     \caption{\textbf{Domain discrepancy in lane detection.} We categorized the cause of domain discrepancy in lane detection. (a) The difference in the number of lanes and curvatures shows a clear discrepancy in lane structures. (b) Judging from the t-SNE~\cite{tsne} analysis, the contextual difference of surroundings is also confirmed.}
%     \label{fig:domain_diff}
% \end{figure}

%% < 앞서 언급했던 문제들과 그것을 어떻게 해결할지에 대한 종합적인 내용 >
In this paper, we propose a novel training framework for generalizing a lane detection model using only a single-source domain.
Firstly, to do this, we decompose the lane detection data into two key elements: lane structures and surroundings.
We achieve domain generalization performance optimized by increasing diversity in each element. 
To enhance diversity in lane structures, we utilize High-Definition (HD) maps with various lane and road information. 
Additionally, we employ generative models to augment diversity in surroundings.
In conclusion, rather than indiscriminately increasing the data, we present a data selection method by identifying a core set among the augmented data, where diversity is maximized.

% ** Contribution
The main contributions of the paper can be summarized as follows:

%%% itemize / abstract / conclusion이랑 마지막에 다시 확인할 것
\begin{itemize}

\item We propose a novel training framework designed to generalize a lane detection model utilizing a single-source domain, addressing the domain generalization challenge in the context of realistic autonomous driving scenarios.

\item We enhance domain generalization performance by systematically increasing diversity in two fundamental elements of lane detection data: lane structures and surroundings. We leveraged HD maps and generative models to enhance diversity in each element.

\item Diverse experimental validations have demonstrated that the proposed training framework outperforms domain adaptation techniques without any prior target domain information.

\end{itemize}

% % 두괄식, 개괄적으로, 주장이 잘 느껴지게(-> 근데 너무 강한 어조로 쓰면 안됨) 
% % 문단과 문단간의 흐름을 생각하면서 !!!!! 
% % [lane & surrounding의 diversity가 중요함] + [이걸 HDMap으로 풀어야 함]

% % -> 이 두개로 나눈 이유 : common한게 아니라 우리의 독특한 '주장'이라는거를 강조해야함 

% % ** lane det 일반론 -> low-level task라 robust 해야함 
% Lane detection is a fundamental task for autonomous driving. 
% It revolves around identifying lane markings or road boundaries, playing a crucial role in assisting autonomous vehicles to stay within drivable areas.
% %% Therefore, lane detection algorithms are mandated to provide consistent and reliable results in any driving circumstances. % 중복된 문장

% %% 이전에는 lane markings characteristic blahblah
% %% 최근 lane detection algorithms들은 data-driven. 눈부신 성능 개선


% % cross evaluation 잘 안됨 -> 현재 generalization에 대한 고려가 부족하다. (주장)
% However, the dynamic and unpredictable driving environment in the real world makes the lane detection model vulnerable. 
% Fig.~\ref{fig:intro}, current state-of-the-art lane detection models are very susceptible to these various causes. 
% %% how and why. 여기서 대략적인 예시를 들면서 lane structure나 surrounding에 대한 운을 띄워야 될까?
% %Judging from 
% %In fact, 
% most research in lane detection is currently focused on improving performance on specific scenarios or benchmark datasets, without addressing the issue of generalization.

% %% Although , 약간의 데이터에 변화에도 모델이 쉽게 vulnerable 해짐
% %% most research in lane detection is currently focused on improving performance on specific scenarios or benchmark datasets
% %% therfore, as shown in fig.1 (a), 다른 대상지역에 대해 평가했을 때 큰 폭의 성능 하락. 
% %%   - 차선의 characteristic이 분명하다는걸 얘기해줘야함. 당연히 다른 domain에서 평가하면 성능이 떨어진다는 얘기가 안나오도록 해야함
% %% 낮/밤의 변화와 같은 풍경의 변화에서부터 심지어 target domain의 차선의 수에 까지 영향을 받는다


% \begin{figure}[!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/ssdg_fig1.eps}
%     \caption{\textbf{The problem and motivation of our method.} (a) We set TUSimple~\cite{tusimple} as the source domain and CULane~\cite{culane} as the target domain to measure the performance. We observed severe performance degradation in various scenes due to the domain shift. All of the performance was measured from GANet~\cite{wang2022keypoint}. (b) In fact, the difference between the two datasets exists in surroundings and lane structures}
%     \label{fig:intro}
% \end{figure}




% % ** 위 문제는 domain shift 때문이라고 기존 연구들에서 많이 지적당해옴. 글고 이를 해결하는 방법은 DA/DG, 특히 SSDG가 있음 + 글고 SSDG는 ld generalization 문제를 푸는데에도 도움이 될 수 있음(주장) 
% % -> 너무 related work처럼 자세히 X 
% Previous studies~\cite{dg1,dg2,dg3,dg4,dg5} have pointed out that domain shift is the cause of generalization performance degradation. 
% %As a way to solve these problems, Domain Adaptation(DA) and Domain Generalization(DG) have been proposed widely. %% 필요 없는 문장
% In particular, Single-Source Domain Generalization(SSDG) aims to generalize to various target domains in a situation where only one source domain is available. This can directly help lane detection generalization in a driving environment where information on the target domain is limited.

% % ** 근데 SSDG에서는 diversity가 중요하다고 알려져있음 + 실제로 lane det에서도 중요함(주장) + 우리 실험이 잘 보여줌 
% % In these SSDG problems, \textit{diversity} enhancement on the source domain is well studied to help generalization.[..] Similarly, we find that diversity enhancement is significant for the effective generalization of lane detection. As can be seen in Fig 2, it can be seen that reducing redundancy of data and training lane detection with various environments helps generalization performance.
% % [Fig.2 : CULane scene 하나씩 늘려가며, TU에서 성능 측정하기, 데이터 개수는 똑같이 맞추기 + 실제로 cu scene 다름 보여주기?] 
% %% 우리 주장이 아님 위의 문단하고 합쳐보자

% % ** 하지만 LD 환경에서 diverse한 data를 취득하기에는 물리적 한계가 있음 (팩트. semi 주장 느낌) 
% %% lane structure와 surrounding을 나누는 얘기를 해야함. SSDG 같은 일반적인 프레임워크만으로는 해결할 수 없다
% Unfortunately, it is physically impossible and costly to acquire data in all possible environments to ensure generalization for all scenarios. 
% Creating a lane detection dataset involves capturing RGB images from vehicle-mounted cameras and annotating lane markings.
% Furthermore, obtaining images in diverse environments requires driving a platform in multiple locations, as well as determining where to acquire data to ensure diversity.






% % ** 따라서 우리는 HDMap을 중심으로 한 novel framework를 제안함 
% Therefore, in this paper, we propose a lane detection training framework using High Definition Maps(HD maps) to minimize the aforementioned physical cost and generate divergent data that helps generalization.
% Our framework can leverage various road and lane information provided in HD maps to construct a dataset for lane detection without the need for manual annotations.
% Moreover, by utilizing an image synthesis model, we can generate a large number of various images, thereby enabling the model to be trained robustly against dynamic lane structures and surroundings in the real world.

% % ** Contribution
% The main contributions of the paper can be summarized as follows:

% \begin{itemize}

% \item We propose the decomposition of the domain gap within the lane detection model: (i) lane structures and (ii) surrounding, and define it as an SSDG problem rather than the existing Domain Adaptation approach for the first time.

% \item We propose a robust lane detection training framework using a generative model that can generate maximum divergence data for lane structures and surroundings. In addition, by using HD maps for the source domain, we propose metrics that can measure the similarity between each lane and its surroundings. Specifically, HD maps can be used for the single source domain to reduce annotation costs and ensure infinite selection fields for lanes and surroundings.

% \item Our experiments outperform existing Domain Adaptation models without target domain information.

% \end{itemize}

% \begin{figure}[!]
%     % \centering
%     \includegraphics[width=0.5\textwidth]{figures/ssdg_fig2.eps}
%     \caption{\textbf{Domain discrepancy in lane detection.} We observed the cause of domain discrepancy in lane detection by dividing it into surrounding and lane structures. (a) Judging from the t-SNE~\cite{tsne} analysis of the images of the two datasets, the contextual difference of surroundings is confirmed. (b) The distribution of the number of lanes and the curvature of the two datasets also show a clear difference.}
%     \label{fig:domain_diff}
% \end{figure}

% % === v 1.5 
% % Lane detection has been widely adopted in the autonomous driving field for detecting lane markings on the roads and localizing drivable spaces. However, the driving environment is usually dynamic and unpredictable. For instance, changes in weather or surrounding environments make the lane detection model vulnerable. In fact, judging from Fig.~\ref{fig:intro}, current state-of-art lane detection models are very susceptible to these various causes. 

% % % These causes have been defined as domain shifts. -> 너무 갑자기 등장한 느낌 

% % \begin{figure}[!]
% %     \centering
% %     \includegraphics[width=0.45\textwidth]{figures/intro_tentative.jpeg}
% %     \caption{(a) means the performance of susceptible state-of-art lane detection models and (b) means domain shifts from lane structures and surroundings within lane detection models}
% %     \label{fig:intro}
% % \end{figure}

% % Specifically, the underlying source of these domain shifts within the lane detection model can be deconstructed into two primary aspects: (i) the lane structure and (ii) the contextual environment. 
% % As illustrated in Fig.~\ref{fig:intro}, diverse surroundings are encountered during data collection in various driving scenarios. In addition, a marked contrast in the lane structure becomes evident when comparing instances of eigenlane representation.\daeun{weak point}

% % Domain Adaptation(DA) and Domain Generalization(DG) methods have been proposed to address the prevailing issue of domain shift. However, the application of DA in real-world driving situations is met with challenges due to its reliance on the target domain. 
% % Although the labeling process is excluded to build the target domain dataset, it is unrealistic to obtain information about all new environments of the driving process in advance. 
% % Furthermore, even in the case of Multi-Source Domain Generalization(MSDG), it is still inefficient because driving data from various sources must be constructed through human annotation. Therefore, in order to build a robust lane detection model that can work practically in the real world, it is necessary to define it in the form of a Single Source Domain Generalization(SSDG) problem.

% % In the SSDG problem, access is confined to only one source domain, so building a methodology that can adapt to other various domains with this limited solitary domain is the main goal. 
% % Thus, it has led to a sufficient discussion on how to narrow the domain gap through \textbf{diversity} improvement. 
% % % For instance, Augmix~\cite{hendrycks2019augmix} and Cutmix~\cite{yun2019cutmix} can be applied in the SSDG field to raise the diversity of the source domain by giving simple pixel-wise noise. 
% % However, the domain shift of the lane detection model is too complicated to be solved by a simple transformation-based method. This is because the semantic domain gap such as lane structure and surrounding generated in a driving environment is insufficient to be narrowed down to simple noise.
% % Nevertheless, diversity is also important for the generalization of the lane detection model. \daeun {a little weak, more is needed}. 
% % Therefore, practical generalization techniques should be required to guarantee diversity for the fact of domain shifts, but it is physically inefficient to directly collect divergent data in a driving environment.

% % % HD map이 여기서 너무 갑자기 튀어 나오는 느낌 
% % In conclusion, we use HD maps to generate diversity-guaranteed data and then use them for training the lane detection model in order to effectively solve domain shifts for lane structure and surrounding within lane detection. 
% % In particular, by using HD map as the source domain rather than the existing benchmark image, it is possible to extract multi-view scenes even at fixed locations to ensure various surrounding. Furthermore, reducing the annotation cost for lanes and obtaining more realistic and diverse lane structures than affine-transformed lane markings can yield tremendous benefits. Our various experiments illustrate the efficiency and excellence of these methods.

% % The main contributions of the paper can be summarized as follows:

% % \begin{itemize}

% % \item We propose the decomposition of the domain gap within the lane detection model: (i) lane structures and (ii) surrounding, and define it as an SSDG problem rather than the existing Domain Adaptation approach for the first time.

% % \item We propose a robust lane detection training framework using a generative model which can generate maximum divergence data for lane structures and surroundings. In addition, by using HD map for the source domain, we propose metrics that can measure the similarity between each lane and its surroundings. Specifically, HD maps can be used for the single source domain to reduce annotation costs and ensure infinite selection fields for lanes and surroundings.

% % \item Our experiments outperform existing Domain Adaptation models without target domain information.

% % \end{itemize}
% % == 

% % 내 주장 : [ Lane structure & surrounding ] + [ HDMap ]
% % Fig 1 = domain shift 그림 (lane, surrounding, 성능 drop) 

% % Lane detection은 자율주행 과정에서 차의 위치를 localization하고 안정적인 주행을 하기 위해 필수적으로 고려되어 왔다. 하지만 자율주행 과정에서 만나는 주행 환경은 매우 dynamic하고 예측하기 어렵다. 예를 들어, 날씨의 변화나 주변 환경의 변화 등은 lane detection 모델의 작동을 취약하게 만든다. 실제로 fig 1으로 미루어 볼 때, 현재 존재하는 state-of-art lane detection 모델들은 이러한 domain shift에 아주 취약하며 이제는 더이상 중요성을 간과할 수 없다. 

% % 특히 lane detection 모델에서 발생하는 domain shift의 원인은 (i) lane structure와 (ii) surrounding으로 decompose 될 수 있다. Structure-texture image decomposition[..]처럼 이미지를 meaningful한 component들로 나누어 고려하는 방법은 고전적으로 이용되어 왔다. Fig 1에서 볼 수 있다시피 데이터가 수집된 주행 환경에 따라 다양한 surrounding이 관찰되며, 이에 따라 eigenlane의 plot처럼 수집되는 lane structure에도 극심한 차이가 있음이 empirical하게 확인된다. 
% % -> \daeun{조금 약한듯 함}

% % 이러한 domain shift를 해결하기 위한 방법으로 현재까지 다양한 domain adaptation, generalization 방법들이 제안되어 왔다.[..] 하지만 target domain의 정보가 요구되는 domain adaptation의 경우 실제 real-world의 주행 상황에서 적용되기 어렵다. 비록 target domain dataset을 구축에서 labeling 과정이 제외되지만, 우리는 주행 과정에 있어 모든 새로운 환경에 대한 정보를 사전에 얻을 수 없기 때문이다. 나아가 multi-source domain generalization의 경우에도 여러 source의 주행 데이터를 human annotation 등의 과정으로 구축해야 하기 때문에 비효율적이다. 따라서 real-world에서 실용적으로 작동할 수 있는 robust한 lane detection 모델의 구축을 위해서는 single source domain generalization(ssdg) 문제 형태로 정의할 필요성이 있다. 

% % SSDG 상황에서는 접근할 수 있는 source domain은 오직 하나이므로, 이러한 한정된 domain으로 다양한 domain에 적응할 수 있는 방법론이 필수적으로 요구된다. 그리고 이는 diversity 향상을 통한 domain gap을 좁히는 방법에 관한 충분한 논의[..]로 이어져왔다. 기존에는 주로 단순한 noise를 부여해 augmentation을 하는 Augmix, Cutmix 등의 방법이 고려되어 왔지만, lane detection 모델의 domain shift는 단순한 transformation-based의 방법으로 해결되기에는 너무 복잡하다. 주행환경에서 발생하는 lane structure와 surrounding 등의 semantic한 domain gap은 단순 noise로 좁혀지기에 불충분하기 때문이다. 
% % 하지만 역시 lane detection 모델의 generalization에도 diversity는 중요하다. + 근거 -> \daeun{조금 약한듯 함. 왜그런지 더 많이 필요}
% % 따라서 lane detection 모델의 실질적인 generalization을 위해서는 각 domain shift 원인에 대해 diversity를 보장할 수 있는 방법이 필요하지만, 주행 환경에서 diverse한 데이터를 직접 수집하기에는 physically impossible하다. 

% % 이러한 상황에서 lane structure와 surrounding에 관한 domain shift를 효과적으로 해결하기 위해 우리는 HD map을 이용해 이들의 diversity가 보장된 데이터를 생성한 후, lane detection model 학습에 이용한다. 특히 기존 밴치마크 image가 아닌 HD map을 source domain으로 사용함으로써 고정된 location에서도 multi-view의 scene을 추출해 다양한 surrounding을 보장할 수 있다. 나아가 lane에 관한 annotation cost를 줄이고, 이미지에서 affine transformation된 lane marking보다 좀 더 realistic하고 다양한 lane structure를 얻을 수 있다. 우리의 여러가지 관찰과 실험들은 이러한 방법의 efficiency와 우수함을 잘 보여준다. 


% % 우리의 contribution은 아래와 같다. 

% % - Real-world 주행환경에서 발생하는 lane detection model의 domain gap의 원인을 lane과 surrounding으로 decompose하고, 최초로 기존 Domain Adaptation의 접근과 달리 조금 더 실용적인 SSDG 문제로 이를 정의한다.

% % - Robust Lane Detection을 위해 HD map을 이용한 lane & surrounding maximal diverse data를 generative model로 생성한 후, 이 중 coreset을 골라 lane detection 학습에 이용하는 framework 제안한다. 특히 여기서 HD map을 사용함으로써 annotation cost를 줄이고, lane과 surrounding에 대한 무한한 selection field를 보장한다. 

% % - 우리의 실험들은 target domain 정보 없이도 기존 domain adaptation 모델들의 성능을 능가한다.


==> src_icra/method.tex <==
\section{Methodology} 

% 8/24 
% -> method가 아직도 좀 서술같은 느낌. 짜임새를 생각해서 다시 구성하면 좋을 듯 
% -> 흐름이 없고 왔다갔다 하는 느낌. 구성
% -> 아예 lane과 surrounding으로 section을 나눠서 각각의 문제에 대해 우리가 문제를 어떻게 풀었다~를 서술하는게 좋음
% -> framework이 약해지는건 어쩔 수 없지 않을까. 이건 그냥 잘 쓰는 수밖에 없음. 
% -> 4.1에서는 pd보다 전체 overview를 설명하고, 4.2 & 4.3에는 관찰에 대해 설명하는게 낫지 않을까 
% -> pd나 selection은 앞으로 빼버리기 

% < 두가지의 큰 갈래 > 
% -> 1) 일반적으로는 novelty가 없을 수도 있지만 DG와 결합되었을 때는 이 framework는 의미가 있다. 이게 특별하게 보이도록 써지는 형태여야 함. 
% -> 2) domain shift가 발생하는 이유를 분석했고, 각각의 이유에 대해서 우리는 이렇게 문제를 풀었다. 

\begin{figure}[!]
    \centering
    \subfloat[]{\includegraphics[width=0.645\linewidth]{figures/fig2-a_v2.pdf}}
    \subfloat[]{\includegraphics[width=0.355\linewidth]{figures/fig2-b_v2.pdf}}
    \caption{\textbf{Domain discrepancy in lane detection.} We categorized the cause of domain discrepancy in lane detection. (a) The difference in the number of lanes and curvatures shows a clear discrepancy in lane structures. (b) Judging from the t-SNE~\cite{tsne} analysis, the contextual difference of surroundings is also confirmed.}
    \label{fig:domain_diff}
    \vspace{-0.4cm} % 와 끗. 일단 가능은 한 것 같으니 제목 이대로 가제출 합니당 -> 일단 vspace 더 조정해놨어요! vspace로는 이게 최선인 것 같습니다 ㅎㅎ..아아 넵넵!! 뺄 문장 찾아볼까요??
    % 가 제출해보니 약간 더 조정할 필요가 있네요. 조금 손보겠습니당
    % 넵 감사합니다!
    % 너무 촘촘한가요? 캡션 한문장 줄이고 싶은데 잘 모르겠네요
\end{figure}

\subsection{Domain discrepancy in lane detection} 
We first explored the cause of domain discrepancy that occurs in lane detection environments. After we observed various factors, we divided the cause of the above domain discrepancy into \textit{(i) lane structures} and \textit{(i) surroundings}. 

For lane structures, we compared the number of lanes included in each scene and curvatures as shown in Fig~\ref{fig:domain_diff}-(a). 
Especially, for detecting lane curvatures, we used the pre-released bezier control points~\cite{feng2022rethinking} to calculate the bezier coefficients which represent the curvature of lanes. 
These plots faithfully demonstrate that the difference in lanes can be one of the factors of the domain discrepancy in lane detection scenarios. 
In addition, as shown in Fig~\ref{fig:domain_diff}-(b), we conducted a t-SNE~\cite{tsne} analysis to observe differences in surroundings. We first extracted image features from ResNet-18 and reduced the dimension via t-SNE. As shown in the result, images from the two datasets form distinctly separate clusters in the feature space. 

% \textbf{Diversity.} Regarding the domain shift above, existing SSDG papers like ~\cite{volpi2018generalizing} mention that diversity is significant. With further study, we observed changes in performance by artificially improving diversity for lane structure and surroundings, respectively. 
% First, for lane structure, the lane of the TUSimple was intentionally transformed into affine transformation, and as a result of training, the performance improvement was confirmed. Furthermore, for surrounding, the performance change in TUSimple was observed by increasing the scene of each category of CULane one by one. As a result, it was observed that the generalization performance for TUSimple improved as the surrounding diversity of CULane increased. 
% This confirms the importance of diversity for the generalization of lane detection empirically.
% In conclusion, the above observation motivates us to introduce diversity maximization techniques that target surroundings and lane structures separately. 

\begin{figure*}[!t]
    \vspace{0.2cm}
    \centering
    \includegraphics[width=0.90\textwidth]{figures/fig3_model.pdf}
    \caption{\textbf{The framework of our method.} Our framework utilizes HD maps and diversity maximization methods to build robust lane detection models. 
    (1) We first extract lane markings from HD maps and project it onto the RGB images to obtain source domain data pairs of images and lane label masks. (2) A generative model is used to synthesize diverse images corresponding to the core set of lane structures with maximal diversity, selected from the source domain data. (3) After again selecting a core set of synthesized images for each lane structure with maximal diversity, (4) we train the lane detection model and obtain enhanced domain generalization performance.
    % We first extract lane markings from HD maps through projection and set it to the source domain. A generative model is used to generate diverse datasets for lane structures and surroundings. 
    }
    \label{fig:fig2_overall_arch}
    \vspace{-2mm}
\end{figure*}

\subsection{Preliminaries}
We propose a framework for enhancing the generalization performance of lane detection models using HD maps and image generation models. 
As shown in Fig.~\ref{fig:fig2_overall_arch}, we describe the proposed framework in several phases. 
We first extract lane markings and images from HD maps and generate realistic scenes to help with training lane detection models. 
At each phase, we try to enhance the diversity of lane structures and surroundings which we consider two main factors for domain discrepancy in lane detection. 

\textbf{Problem definition.}
For the Single-Source Domain Generalization(SSDG) setting for lane detection, we use source domain dataset ${D_s}$ which consists of pairs of driving environment image and lane marking. 
Our work demonstrates HD maps can be a successful source domain for mitigating domain discrepancy in lane detection environments. 
To train the lane detection model as robustly as possible for the several unseen target domains ${D_t}$, we propose a diversity-targeted framework by using HD maps. More specifically, we extract the core set ${D_s^*}$ of augmented samples maximizing the diversity of surroundings and lane structures. 
%which are aforementioned for the factor of domain discrepancy. 

\textbf{Data selection algorithm.}  % 단순하지만, 최적 해를 보장?하고 다양한 형태의 데이터에 similarity metric만 정하면 적용할 수 있음 (우리의 경우 lane, surrounding에 적용가능한 방법이 필요했음) 
In this paper, we define \textit{maximal diversity} as \textit{minimum sum of similarities} between nodes in a graph.
Let's assume a complete weighted graph $G=(V, E, W)$ where the vertex set $V=\{v_1, v_2, ..., v_N\}$ represents $N$ data points, and each data point is connected to every other data point through an edge $E=\{(v_i, v_j)\}$. The weight of each edge $W=\{w(i,j)\}$ is defined as the similarity between the two data points connected by the edge. The near-optimal solution can be configured as Algorithm~\ref{alg:search_algo}.   % 방법론 
This can be freely applied to various types of data by defining only a simple metric, so it can be applied regardless of lane structure and surrounding image.   % 우리 방법에 좋은 이유 
Next, we define each of the similarity functions to utilize for maximal diversity selection below.

% 어렵네용 ㅎㅎ.. 
% 헉 무슨방법인가용 ㅋㅋ 아아 그렇군요! 
% 이상한 방법들은 알고 있는데 그러면 다른 문제가 더 커질까봐... minipage같은거 만들어서 넣는 방법이 있거든요. 일단 이것저것 다른 것 조금 더 해보겠습니당!
% \begin{algorithm}[t]
% % \footnotesize 
% \small
% \caption{Finding a set of K vertices \newline with the minimum sum of similarity}
% \begin{algorithmic}[1]
% \Require Complete weighted graph $G$ and $K=\#$ of vertices
% \State Find the vertex pair $(i,j)$ which has minimum $w(i, j)$
% \State Add $i$ and $j$ to $Q$
% \While{$|Q| < K$}
% \State Find vertex $k$ which minimizes $\sum_{l \in V \setminus Q} w(k, l)$
% \EndWhile
% \Ensure $Q$
% \end{algorithmic}
% \label{alg:search_algo}
% \end{algorithm}


\subsection{Increasing the diversity of lane structures}
\textbf{Lane mask extraction from HD map.} We especially leverage the lane-related information in HD maps to construct our framework. Using the camera parameters of pre-built HD maps, we can generate the lane label masks by projecting the lane objects in HD maps within the camera view at the current location onto the camera image plane. It is worth noting that this process does not require any additional annotation to obtain the pixel-level positions of the lane markings on the image plane. 
Therefore, we can acquire a substantial number of lane-label masks from HD maps.


\textbf{Selection with lane structures similarities.} We propose a lane similarity function $s$ between two lane label masks $\textbf{M}_i, \textbf{M}_j$ that can take into account the number of lanes and curvature. 
We first simplify the problem by defining the similarity between the projections of each lane mask $\ell$ onto the image plane. We plan to use the method proposed by \cite{eigenlane} to compare the similarity between lane curves represented in pixel coordinates. 
% 여기에 eigenlane 장점 들어가면 좋을 듯? 

First, we express a lane as a set of 2D points uniformly sampled along the vertical direction in the image plane, i.e., $\ell=[x_1, x_2, ..., x_N]^T$, where $x_i$ denotes the $x$-coordinate of the $i$-th sample, and $N$ is the number of samples. 
We construct a lane matrix $\textbf{A}=[\ell_1, \ell_2, ..., \ell_L]$ by utilizing all $L$ lane curves from the entire training data. By applying the SVD algorithm to the constructed lane matrix $\textbf{A}$, we can factorize it as follows:
\begin{equation}
   \textbf{A}= \textbf{U} \Sigma \textbf{V}^T,
\end{equation}
where $\textbf{U}=[\textbf{u}_1, ..., \textbf{u}_N]$ and $\textbf{V}=[\textbf{v}_1, ..., \textbf{v}_L]$ are orthogonal matrices, and $\Sigma$ is a singular value matrix. 
Therefore, each lane curve $\ell$ can be approximated using $M$-rank approximation with singular vectors $\textbf{u}_1, ..., \textbf{u}_M$ as follows:
\begin{equation}
\tilde{\ell_i} = \textbf{U}_M \textbf{c}_i = [\textbf{u}_1, ..., \textbf{u}_M] \textbf{c}_i.
\end{equation}

The coefficient vector $\textbf{c}_i$ of each lane curve $\ell_i$ in the \textit{eigenlane} space spanned by the singular vectors $[\textbf{u}_1, ..., \textbf{u}_M]$ can be expressed as follows:
\begin{equation}
\textbf{c}_i = \textbf{U}_{M}^{T} \ell_i = [c_1, ..., c_M].
\end{equation}

Therefore, we simply define the similarity between two lane curves $\ell_i$ and $\ell_j$ as Euclidean distance by projecting onto the \textit{eigenlane} space as follows:
\begin{equation}
d(\ell_i, \ell_j) = | \textbf{c}_i - \textbf{c}_j |.
\end{equation}

Our goal is to extend the similarity between lane curves to between lane label masks.
Given two lane label masks $\textbf{M}_i=[\ell_{0}^{i}, ..., \ell_{m}^{i}]$ and $\textbf{M}_j=[\ell_{0}^{j}, ..., \ell_{n}^{j}]$, each containing $m$ and $n$ lane curves, respectively.
Assuming that $m\ge n$ always holds, we define the lane layout similarity $s$ between lane label marks $\textbf{M}_i, \textbf{M}_j$ as follows: 
\begin{equation}
  s(\textbf{M}_i, \textbf{M}_j) = \sum^{n}_{k} \min_{l}  d( \ell_{l}^{i}, \ell_{k}^{j} )  + |m-n|~\kappa,
\end{equation}
where $\kappa$ denotes the penalty constant which we describe next. 
We believe that the number of curves is also an important factor in determining the similarity. 
Therefore, when the two-lane label masks have different numbers of lane curves, we penalize their similarity by adding $\kappa$.
We empirically determine the penalty constant $\kappa$ from the training dataset.
This indicates that we consider the number of lane curves to be an important factor affecting diversity in most cases. With the definition of similarity between lane label masks, we can select the $K_{\text{scene}}$ number of masks that maximize the diversity of lane layouts by using the selection algorithm in Algorithm~\ref{alg:search_algo}.

\begin{algorithm}[t]
% \footnotesize 
\small
\caption{Finding a set of K vertices \newline with the minimum sum of similarity}
\begin{algorithmic}[1]
\Require Complete weighted graph $G$ and $K=\#$ of vertices
\State Find the vertex pair $(i,j)$ which has minimum $w(i, j)$
\State Add $i$ and $j$ to $Q$
\While{$|Q| < K$}
\State Find vertex $k$ which minimizes $\sum_{l \in V \setminus Q} w(k, l)$
\EndWhile
\Ensure $Q$
\end{algorithmic}
\label{alg:search_algo}
\end{algorithm}


\subsection{Increasing the diversity of surroundings}
% \textbf{Image scene extraction from HD map.}     % image extraction..? 

\textbf{Selection with surrounding similarities.}
Our expectation is that by training the model with RGB images having identical lane labels, but different surroundings and backgrounds, the model will be less sensitive to changes in the backgrounds and surroundings. However, unlike the case of lane layouts, it is difficult to obtain a quantitative measure of the similarity between backgrounds or surroundings in RGB images. 
Therefore, we use a comparison metric commonly used to check the quality of generated images by image synthesis models.
Therefore, we define the similarity of the surroundings in RGB images as an image metric. 

% SSIM이 적합한 이유 -> 보완 필요 
The structural similarity index measure (SSIM)~\cite{ssim} and its multi-scale extension (MS-SSIM)~\cite{ms-ssim} is a method used to compare the perceived quality of digital images and videos. They are commonly used for measuring the similarity between two images. 
Recently, MS-SSIM has also been used to compare the quality of generated images against the reference images in image generation tasks~\cite{snell2017learning}. 
Therefore, we can choose the MS-SSIM as the similarity metric between two generated images.     

Finally, to train the lane detection model, we generate 100 RGB images for each lane label mask and we selected $K_{\text{image}}$ most perceptively diverse set of generated images using MS-SSIM and the method described in Algorithm~\ref{alg:search_algo}.



==> src_icra/related.tex <==
% < 1. Domain Adaptation w/ Lane Detection > - O 


\section{Related Works}

\subsection{Domain Adaptation for Lane Detection} 
Unsupervised Domain Adaptation(UDA)~\cite{uda1,uda2,uda3,uda4} has been primarily adopted as a methodology for bridging domain discrepancy that occurs between different domains. In fact, it allows access to unlabeled target domains in the model learning process. Current research for domain adaptation in lane detection can be largely categorized into (i) Sim-to-Real and (ii) Cross-domain adaption. 

(i) \textbf{Sim-to-Real domain adaptation} is a field that adapts simulated data generated by gaming engines to the real world. Their main goal is to bridge the domain gap between photorealistic synthetic images and real-world data. ADA~\cite{simada} utilizes adversarial discriminative and generative methods for adapting to the target domain, and UNIT~\cite{simunit} utilizes cycle-GAN-based methods. 

(ii) \textbf{Cross-domain adaptation} is a method for narrowing the domain gap that occurs in two different driving environments. MLDA~\cite{li2022multi} is the first paper to point out the cross-domain discrepancy among CULane and TUSimple datasets. They solve this domain gap with a framework based on self-training.
In particular, the setting of MLDA is also a form of cross-evaluation with only one source domain. However, the biggest difference from our framework is that they use RGB images of the target domain in their adaptation process.

Given that both of the above fields require target domain information, it is difficult to apply it in a realistic driving environment.

% < 2. Single-Source Domain Generalization > 
\subsection{Single-Source Domain Generalization} 
Unlike Multi-Source Domain Generalization(MSDG), Single-Source Domain Generalization(SSDG)~\cite{ssdg1,ssdg2,ssdg3} utilizes only one source domain during training. Intuitively, SSDG is more difficult to generalize successfully than MSDG because of the limited training situations. 
Existing SSDG models have been developed by applying data augmentation techniques to the source domain and expecting to make a robust dataset~\cite{su2023rethinking,wang2021learning,volpi2018generalizing,qiao2020learning}. 
The landmark works are ADA~\cite{volpi2018generalizing} and M-ADA~\cite{qiao2020learning}, which use adversarial data augmentation techniques to conduct pixel-level additive perturbation. 

On top of that, the maximization of diversity has been widely explored to boost generalization effects.~\cite{wang2021learning,wacv23diverse,zhang2019adversarial,hendrycks2019augmix, yun2019cutmix} % citation
ALT~\cite{wacv23diverse} produces diverse images using a separate diversity module that combines augmentation such as Augmix~\cite{hendrycks2019augmix} and RandConv~\cite{randconv}.
However, from the standpoint of lane detection fields, these augmentation techniques are insufficient to contain a complex and dynamic driving environment. Therefore, in this work, we propose a method of selecting a core set that can maximize the diversity of lane structures and surroundings for generalizing lane detection models.
%as part of a more advanced augmentation method.



% < 3. HD map > -> \daeun{HDmap의 background / lane structure에서의 장점이 추가되면 좋을 것 같다.}
\subsection{HD maps}     
HD maps are widely recognized for their ability to provide accurate and detailed semantic information about road environments in a machine-readable form.
Despite being represented in a lightweight vector map format, HD maps contain detailed and accurate information about the road environment. 
This information is primarily used for vehicle localization and control~\cite{hdmap_loc}. 
Recently, there has been a growing interest in the rich semantic information contained in HD maps, and several studies~\cite{hdmap_trajpred, hdmap_cd2, hdmap_gen1} have utilized them for various other tasks beyond localization and control. 
Similarly, our study also utilizes road information from HD maps to improve the generalization performance of lane detection. 
